A Cartesian Bicategory of Polynomial Functors in Homotopy Type Theory

Polynomial functors are a categorical generalization of the usual notion of polynomial, which has found many applications in higher categories and type theory: those are generated by polynomials consisting a set of monomials built from sets of variables. They can be organized into a cartesian bicategory, which unfortunately fails to be closed for essentially two reasons, which we address here by suitably modifying the model. Firstly, a naive closure is too large to be well-defined, which can be overcome by restricting to polynomials which are finitary. Secondly, the resulting putative closure fails to properly take the 2-categorical structure in account. We advocate here that this can be addressed by considering polynomials in groupoids, instead of sets. For those, the constructions involved into composition have to be performed up to homotopy, which is conveniently handled in the setting of homotopy type theory: we use it here to formally perform the constructions required to build our cartesian bicategory, in Agda. Notably, this requires us introducing an axiomatization in a small universe of the type of finite types, as an appropriate higher inductive type of natural numbers and bijections.

==> abstract.tex <==
In order to gain a better understanding of the state space of programs, with the
aim of making their verification more tractable, models based on directed
topological spaces have been introduced, allowing to take in account equivalence
between execution traces, as well as translate features of the execution (such
as the presence of deadlocks) into geometrical situations. In this context, many
algorithms were introduced, based on a description of the geometrical models as
regions consisting of unions of rectangles. We explain here that these
constructions can actually be performed directly on the syntax of programs, thus
resulting in representations which are more natural and easier to implement. In
order to do so, we start from the observation that positions in a program can be
described as partial explorations of the program. The operational semantics
induces a partial order on positions, and regions can be defined as formal
unions of intervals in the resulting poset. We then study the structure of such
regions and show that, under reasonable conditions, they form a boolean algebra
and admit a representation in normal form (which corresponds to covering a space
by maximal intervals), thus supporting the constructions needed for the purpose
of studying programs. All the operations involved here are given explicit
algorithmic descriptions.

% Verification of concurrent programs is notoriously hard, even for simple
% programs and has introduced many fascinating theories linking topology to
% programs and their execution. In this paper we explore a different take on the
% representations of paths and execution of programs, dismissing geometric
% realization to focalise on a discrete representation of partial execution to
% define the poset corresponding to the state space of our programs. Our goal is
% to study the underlying structure of such poset and under which conditions we
% can define canonical finite representations of the subset of explorations, and
% verifiable conditions for their existence. These canonical representation are
% made to correspond to cover by maximal cubes for precubical sets, expanding
% previous methods by allowing infinite unwrapping of loops.


==> eptcsdata.tex <==
\providecommand{\firstpage}{67}
\providecommand{\publicationstatus}{Ana Sokolova (Eds.): MFPS 2021\\
EPTCS 351, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.351.5}{10.4204/EPTCS.351.5}}
\pdfoutput=1

